Performance comparison of Dask and Apache Spark on HPC systems for Neuroimaging

The general increase in data size and data sharing motivates the adoption of Big Data strategies in several scientific disciplines. However, while several options are available, no particular guidelines exist for selecting a Big Data engine. In this paper, we compare the runtime performance of two popular Big Data engines with Python APIs, Apache Spark, and Dask, in processing neuroimaging pipelines. Our experiments use three synthetic \HL{neuroimaging} applications to process the \SI{606}{\gibi\byte} BigBrain image and an actual pipeline to process data from thousands of anatomical images. We benchmark these applications on a dedicated HPC cluster running the Lustre file system while using varying combinations of the number of nodes, file size, and task duration. Our results show that although there are slight differences between Dask and Spark, the performance of the engines is comparable for data-intensive applications. However, Spark requires more memory than Dask, which can lead to slower runtime depending on configuration and infrastructure. In general, the limiting factor was the data transfer time. While both engines are suitable for neuroimaging, more efforts need to be put to reduce the data transfer time and the memory footprint of applications.

==> Lato-fonts/Makefile <==
## Makefile
## Copyright 2011 Mohamed El Morabity
#
# This work may be distributed and/or modified under the conditions of the LaTeX
# Project Public License, either version 1.3 of this license or (at your option)
# any later version. The latest version of this license is in
# http://www.latex-project.org/lppl.txt and version 1.3 or later is part of all
# distributions of LaTeX version 2005/12/01 or later.
#
# This work has the LPPL maintenance status `maintained'.
#
# The Current Maintainer of this work is Mohamed El Morabity
#
# This work consists of all files listed in manifest.txt.

######################
# Fonts informations #
######################

FONT_NAME = lato
FOUNDRY = public
FONT_CODES = fla

# Supported LaTeX encodings
SUPPORTED_ENCODINGS = ot1 t1 ts1
# Supported LaTeX encodings containing small caps
SUPPORTED_SC_ENCODINGS = $(filter-out ts1,$(SUPPORTED_ENCODINGS))
# Custom encodings provided
INPUT_ENCODINGS = $(INPUT_ETX_FILES:$(FONT_NAME)-%.etx=%)


#####################
# Installation root #
#####################

TEXMFHOME = $(shell kpsexpand '$$TEXMFHOME')


###########
# Archive #
###########

ARCHIVE_ROOT = $(FONT_NAME)
ARCHIVE = $(FONT_NAME).zip


###########
# Sources #
###########

TRUETYPE_FILES = $(wildcard *.ttf)

# Fontinst files
FONTINST_FILE = $(FONT_NAME)-drv.tex
FONTINST_MAP_FILE = $(FONT_NAME)-map.tex

# Custom Fontinst encoding files
INPUT_ETX_FILES = $(FONT_NAME)-01.etx $(FONT_NAME)-02.etx $(FONT_NAME)-dotlessj.etx
MTX_FILES = $(FONT_NAME)-fixlatin.mtx $(FONT_NAME)-fixtextcomp.mtx

STYLE_FILES = $(wildcard *.sty)

DOCUMENTATION = $(FONT_NAME).tex $(FONT_NAME).pdf $(FONT_NAME)-samples.tex $(FONT_NAME)-samples.pdf README CHANGES

# Files to be installed in texmf/source
SOURCE_FILES = $(FONTINST_FILE) $(FONTINST_MAP_FILE) $(INPUT_ETX_FILES) $(MTX_FILES) Makefile ttf2type1.pe


###################
# Generated files #
###################

TYPE1_FILES = $(TRUETYPE_FILES:.ttf=.pfb) $(TRUETYPE_FILES:.ttf=-LCDFJ.pfb)
AFM_FILES = $(TYPE1_FILES:.pfb=.afm)

# Fontinst log file
FONTINST_REC_FILE = $(FONT_NAME)-rec.tex

# Metrics files
PL_FILES = $(foreach e,$(INPUT_ENCODINGS),   \
             $(TRUETYPE_FILES:.ttf=-$(e).pl) \
           )
OUTPUT_MTX_FILES = $(PL_FILES:.pl=.mtx)
VPL_FILES = $(foreach e,$(SUPPORTED_ENCODINGS),          \
              $(TRUETYPE_FILES:.ttf=-$(e).vpl)           \
            )                                            \
            $(foreach e,$(SUPPORTED_SC_ENCODINGS),       \
              $(TRUETYPE_FILES:.ttf=-SmallCaps-$(e).vpl) \
            )
TFM_FILES = $(PL_FILES:.pl=.tfm) $(VPL_FILES:.vpl=.tfm)
VF_FILES = $(VPL_FILES:.vpl=.vf)

MAP = $(FONT_NAME).map

# Font definition files
FD_FILES = $(foreach e,$(SUPPORTED_ENCODINGS), \
             $(foreach f,$(FONT_CODES),        \
               $(e)$(f).fd                     \
             )                                 \
           )

# Generated encoding files
ENC_FILES = $(INPUT_ETX_FILES:.etx=.enc)

# Generated files to be installed
GENERATED_FILES = $(TYPE1_FILES) $(AFM_FILES) $(TFM_FILES) $(VF_FILES) $(MAP) $(FD_FILES) $(ENC_FILES)


default: all


all: dist


dist: $(ARCHIVE)


%.pfb %.afm: %.ttf
	fontforge ttf2type1.pe $<
	# BUGFIX: fix FontName to the name of the file
	sed -i "s/^FontName .*/FontName $*/" $*.afm


%-LCDFJ.pfb: %.pfb
	t1dotlessj $< $@


%-LCDFJ.afm: %-LCDFJ.pfb
	pf2afm $<
	# BUGFIX: fix FontName to the name of the file
	sed -i "s/^FontName .*/FontName $*/" $*.afm


%.tfm: %.pl
	pltotf $< $@


%.tfm: %.vpl
	vptovf $^ $


%.vf: %.vpl
	vptovf $^ $@


$(FONTINST_REC_FILE): $(AFM_FILES) $(MTX_FILES) $(FONTINST_FILE)
	latex $(FONTINST_FILE)


$(PL_FILES) $(VPL_FILES): $(FONTINST_REC_FILE)


$(MAP): $(FONTINST_REC_FILE) $(FONTINST_MAP_FILE)
	latex $(FONTINST_MAP_FILE)


$(FD_FILES) $(ENC_FILES): $(MAP)


texmf-tree: clean-texmf-tree $(GENERATED_FILES) $(SOURCES_FILES)
	mkdir -p $(ARCHIVE_ROOT)/doc/fonts/$(FONT_NAME)/
	mkdir -p $(ARCHIVE_ROOT)/tex/latex/$(FONT_NAME)/
	mkdir -p $(ARCHIVE_ROOT)/fonts/{enc,map}/dvips/$(FONT_NAME)/
	mkdir -p $(ARCHIVE_ROOT)/fonts/{afm,tfm,truetype,type1,vf}/$(FOUNDRY)/$(FONT_NAME)/
	mkdir -p $(ARCHIVE_ROOT)/source/fonts/$(FONT_NAME)/
	cp -p $(DOCUMENTATION) $(ARCHIVE_ROOT)/doc/fonts/$(FONT_NAME)/
	cp -p $(FD_FILES) $(STYLE_FILES) $(ARCHIVE_ROOT)/tex/latex/$(FONT_NAME)/
	cp -p $(ENC_FILES) $(ARCHIVE_ROOT)/fonts/enc/dvips/$(FONT_NAME)/
	cp -p $(MAP) $(ARCHIVE_ROOT)/fonts/map/dvips/$(FONT_NAME)/
	cp -p $(AFM_FILES) $(ARCHIVE_ROOT)/fonts/afm/$(FOUNDRY)/$(FONT_NAME)/
	cp -p $(TFM_FILES) $(ARCHIVE_ROOT)/fonts/tfm/$(FOUNDRY)/$(FONT_NAME)/
	cp -p $(TRUETYPE_FILES) $(ARCHIVE_ROOT)/fonts/truetype/$(FOUNDRY)/$(FONT_NAME)/
	cp -p $(TYPE1_FILES) $(ARCHIVE_ROOT)/fonts/type1/$(FOUNDRY)/$(FONT_NAME)/
	cp -p $(VF_FILES) $(ARCHIVE_ROOT)/fonts/vf/$(FOUNDRY)/$(FONT_NAME)/
	cp -p $(SOURCE_FILES) $(ARCHIVE_ROOT)/source/fonts/$(FONT_NAME)/
	cp -p README $(ARCHIVE_ROOT)
	cd $(ARCHIVE_ROOT) && find . -type f > manifest.txt


$(ARCHIVE): clean-texmf-tree texmf-tree
	zip -r $@ $(ARCHIVE_ROOT)


install: texmf-tree
	mkdir -p $(TEXMFHOME)
	cp -a $(ARCHIVE_ROOT)/* $(TEXMFHOME)
	texhash
	updmap --enable Map=$(MAP)


uninstall:
	$(RM) -r $(TEXMFHOME)/doc/latex/$(FONT_NAME)/
	$(RM) -r $(TEXMFHOME)/tex/latex/$(FONT_NAME)/
	$(RM) -r $(TEXMFHOME)/fonts/{enc,map}/dvips/$(FONT_NAME)/
	$(RM) -r $(TEXMFHOME)/fonts/{afm,tfm,type1,vf}/$(FOUNDRY)/$(FONT_NAME)/
	$(RM) -r $(TEXMFHOME)/source/$(FONT_NAME)/
	updmap --disable $(MAP)
	texhash


clean: clean-texmf-tree
	$(RM) $(TYPE1_FILES) $(AFM_FILES)
	$(RM) $(FONTINST_REC_FILE)
	$(RM) $(PL_FILES) $(TYPE1_FILES:.pfb=.pl)
	$(RM) $(OUTPUT_MTX_FILES) $(TYPE1_FILES:.pfb=.mtx)
	$(RM) $(VPL_FILES)
	$(RM) $(TFM_FILES)
	$(RM) $(VF_FILES)
	$(RM) $(MAP)
	$(RM) $(FD_FILES)
	$(RM) $(ENC_FILES)
	$(RM) $(ARCHIVE)
	$(RM) *~ *.log


clean-texmf-tree:
	$(RM) -r $(ARCHIVE_ROOT)


.PHONY: clean clean-texmf-tree texmf-tree

